Equivariant and Stable Positional Encoding for More Powerful Graph Neural Networks

Graph neural networks (GNN) have shown great advantages in many graph-based learning tasks but often fail to predict accurately for a task-based on sets of nodes such as link/motif prediction and so on. Many works have recently proposed to address this problem by using random node features or node distance features. However, they suffer from either slow convergence, inaccurate prediction, or high complexity. In this work, we revisit GNNs that allow using positional features of nodes given by positional encoding (PE) techniques such as Laplacian Eigenmap, Deepwalk, etc. GNNs with PE often get criticized because they are not generalizable to unseen graphs (inductive) or stable. Here, we study these issues in a principled way and propose a provable solution, a class of GNN layers termed PEG with rigorous mathematical analysis. PEG uses separate channels to update the original node features and positional features. PEG imposes permutation equivariance w.r.t. the original node features and imposes $O(p)$ (orthogonal group) equivariance w.r.t. the positional features simultaneously, where $p$ is the dimension of used positional features. Extensive link prediction experiments over 8 real-world networks demonstrate the advantages of PEG in generalization and scalability.

==> 700-oldprelim.tex <==
\section{Notations and Preliminaries}
%This section introduces relevant materials about graph neural network and permutation equivariance, which will be utilized in the description of our method.

%\pan{Notations: You need to have enough notation setup to introduce GNN and permutation equivariance. Also, discuss a little bit why permutation equivariance is important.}
%\pan{I do not think you need to introduce translation \& rotation equivariance. We just focus on orthogonal group.}

%\pan{Define degree $D$, define expectation, define eigenvalue decomposition, and }

In this section, we prepare the notations and preliminaries that are useful later. First, we define graphs.

\begin{definition}[Graph] Unless specified, we always consider undirected graphs of $N$ nodes and let $[N]=\{1,2,...,N\}$. One such graph can be denoted as $\gG=(A,X)$, where $A$ is the adjacent matrix. $X\in\mathbb{R}^{N\times F}$ denotes the node features, where the $v$th row, $X_v$ is the feature of node $v$. The graph may have self loops, i.e., $A$ has nonzero diagonals. Denote $D$ as the diagonal degree matrix where the diagonal $D_{vv}=\sum_{u\in[N]}A_{vu}$ for $v\in[N]$. %Denote a degree normalized adjacency matrix with a self-loop as $\hat{A} = (A + I)$
Denote the normalized adjacency matrix as $\hat{A}=D^{-\frac{1}{2}}AD^{-\frac{1}{2}}$ and the normalized Laplacian matrix as $L=I-\hat{A}$.
\end{definition}

\begin{definition}[Permutation] An $N$-dim permutation matrix $P$ is a matrix in $\{0,1\}^{N\times N}$ where each row or each column has only one single 1. All such matrices are collected in $\Pi(N)$, simplied as $\Pi$.
\end{definition}

We may adopt the Frobenius norm $\|\cdot\|_\text{F}$ or operator norm $\|\cdot\|_\text{op}$ to measure the matrix distance. 

\begin{definition}[Graph-matching] Given two graphs $\gG^{(i)}=(A^{(i)},X^{(i)})$ and their normalized Laplacian matrices $L^{(i)}$ for $i\in\{1,2\}$, their matching can be denoted by a permutation matrix $P\in \Pi$ that best aligns the graph structures and the node features. 
\begin{align*}
    P^{*}(\gG^{(1)}, \gG^{(2)}) \triangleq \argmin_{P\in \Pi}  \|L^{(1)} - PL^{(2)}P^T\|_{\text{F}} + \| X^{(1)} - PX^{(2)}\|_{\text{F}}
\end{align*}
Using $L$ instead of $A$ to represent graph structure is for notational simplicity. Actually for an unweighted graph, there is a bijective mapping between $L$ and $A$. One can rewrite the first term with $A$. Later, we use $P^*$ by not specifying $\gG_1$ and $\gG_2$ if there is no confusion. The distance between the two graphs can be defined as $d(\gG_1, \gG_2) = \|L^{(1)} - P^*L^{(2)}P^{*T}\|_{\text{F}} + \| X^{(1)} - P^*X^{(2)}\|_{\text{F}}$.
\end{definition}

Next, review eigenvalue decomposition and summarize the arguments on its uniqueness in Lemma~\ref{thm:evd}. 

\begin{definition}[Eigenvalue Decomposition (EVD)] \label{def:evd}
For a positive semidefinite (PSD) matrix $B\in \mathbb{R}^{N\times N}$, it has eigenvalue decomposition $B=U\Lambda U^T$ where $\Lambda$ is a real diagonal matrix with the eigenvalues of $B$ as its diagonal components $0\leq \lambda_1 \leq \lambda_2\leq ... \leq \lambda_N$. $U = [u_1, u_2,...,u_N]$ is an orthogonal matrix where $u_i\in\mathbb{R}^N$ is the $i$th eigenvector, i.e. $Bu_i =\lambda_i u_i$.
\end{definition}

\begin{definition}[Orthogonal Group in the Euclidean space]
$\text{SO}(k) =\{Q\in \mathbb{R}^{k\times k}| QQ^T = Q^TQ= I\}$ includes all $k$-by-$k$ orthogonal matrices. A subgroup of $\text{SO}(k)$ includes all diagonal matrices with $\pm1$  as the diagonal components, $\text{SN}(k) = \{Q\in \mathbb{R}^{k\times k}| Q_{ii}\in\{-1,1\}, Q_{ij} = 0, \, \text{for}\, i\neq j\}$.
\end{definition}
%$I$ is the identity matrix.
%\textbf{Definition 2.4} (Orthogonal group) A $n \times n$ matrix is an orthogonal matrix if $AA^T = I$, where $A^T$ is the transpose of $A$ and $I$ is the identity matrix. For every $n>0$, since the $n \times n$ orthogonal matrices are closed under multiplication and taking inverses, they form the orthogonal group $SO(n)$. 

%Note that EVD is not unique due to the following theorem.

\begin{lemma} \label{thm:evd}
 EVD is not unique. If all the eigenvalues are distinct, i.e., $\lambda_i\neq \lambda_j$, $U$ is unique up to the signs of its columns, i.e., replacing $u_i$ by $-u_i$ also gives EVD. If there are multiple eigenvalues, say $\lambda_{i-1}< \lambda_i = \lambda_{i+1} =...=\lambda_{i+k-1} < \lambda_{i+k}$, then $[u_i, u_{i+1}, ...,u_{i+k-1}]$ lies in an orbit induced by the orthogonal group $\text{SO}(k)$, i.e., replacing $[u_i, u_{i+1}, ...,u_{i+k-1}]$ by $[u_iQ, u_{i+1}Q, ...,u_{i+k-1}Q]$ for any $Q\in \text{SO}(k)$ where keeping other eigenvalues unchanged also corresponds to EVD.
\end{lemma}

Next, we define Positional encoding (PE). PE is the class of techniques to associate each node in the graph with a dense vector in a metric space where the distance between two vectors can represent the distance between their corresponding nodes in the graph. %Traditional network embeddings all provide effective positional encoding techniques~\citep{belkin2003laplacian,tang2015line,perozzi2014deepwalk,grover2016node2vec}. 
\begin{definition}[Positional Encoding]
Given a graph $\gG = (A, X)$, PE works on $A$ and gives $Z=\text{PE}(A)\in\mathbb{R}^{N\times p}$ where each row $Z_v$ gives the positional feature of node $v$.
\end{definition}
The absolute values given by PE may not be useful while the distances between the positional features are more relevant. So, we define PE-matching that allows rotation and translation to best match positional features, which further defines the distance between two collections of positional features. Later, we use $\mathbf{1}\in\mathbb{R}^{N}}$ to denote the all 1 vector and by default assume all vectors are vertical. 
%For most downstream tasks, the absolute values of positional features may not useful while the distances between the positional features are more relevant. To measure the distance between two groups of positional features, we need to define PE-matching that allows rotate and translate positional features.    
\begin{definition}[PE-matching] \label{def:pe-matching}
Consider two groups of positional features $Z^{(1)},\, Z^{(2)}\in\mathbb{R}^{N\times p}$. Their matching is denoted given by $(Q^*(Z^{(1)}, Z^{(2)}), b^*(Z^{(1)}, Z^{(2)}))\triangleq \argmin_{Q\in \text{SO}(p), b\in \mathbb{R}^p}\|Z^{(1)} - Z^{(2)}Q - \mathbf{1}b^T\|_{\text{F}}$. Later, $Q^*,\,b^*$ will be used if caused no confusion. Then, define the distance between two groups of positional features as $\eta(Z^{(1)}, Z^{(2)}) = \|Z^{(1)} - Z^{(2)}Q^*- \mathbf{1}b^{*T}\|_{\text{F}}$.  
\end{defition}


%\begin{definition}[Subspace Distance]
%Consider two matrices $U^{(i)}\in \mathbb{R}^{N\times k}$, $i=1,2$. Their column space distance is defined as $\|U^{(1)}U^{(1)T} - U^{(2)}U^{(2)T}\|_\text{F}$. 
%subspaces in $\mathbb{R}^N$. Suppose their one orthogonal basis can be denoted by $U$ and $U$  
%\end{defition}

\hide{
Let $D$ be the diagonal degree matrix and define $\hat{A}= \frac{D}^{-\frac{1}{2}}(A + I)\frac{D}^{-\frac{1}{2}}$ 


where $V$ is the set of $n=|V|$ nodes, $E$ is the set of edges in $V \times V$. $X \in \mathbb{R}^{n \times k}$ denote the node features, where the $v$th row, $X_v$ denotes the features of node $v \in V$. Since graphs are usually sparse, the adjacent matrix $A \in \{0,1\}^{n \times n}$is introduced to describe a graph $G$. If an edge $(u,v)$ exists in $E$, $A_{uv}=1$. Thus, we can also denote $\gG=(A,X)$.                         

\textbf{Definition 2.2} (Permutation action $\pi$). We define $\pi$ as a bijective mapping from $V$ to $V$, which can acts on any vector or tensor defined by nodes $V$. All such permutation actions $\pi$ are collected in the set $\Pi_n$.

\textbf{Definition 2.3} (Permutation equivariance). We define $T_g$ : $X \rightarrow X$ as a set of transformations on group $g \in \gG$ and $S_g$ as an equivalent transformation on the output space $Y  \rightarrow Y$. We say a function $\phi$ : $X \rightarrow Y$ is equivalent to $g$ if $\phi(T_g(x)) = S_g(\phi(x))$. If a function $f$ is Permutation equivariance, permuting the input results in the same permutation of the output of $f$, such as: $f(\pi(x)) = \pi(f(x))$, where $\pi \in \Pi$ is a permutation action. 

\textbf{Definition 2.4} (Orthogonal group) A $n \times n$ matrix is an orthogonal matrix if $AA^T = I$, where $A^T$ is the transpose of $A$ and $I$ is the identity matrix. For every $n>0$, since the $n \times n$ orthogonal matrices are closed under multiplication and taking inverses, they form the orthogonal group $O(n)$. 

\textbf{Definition 2.5} (Graph representation learning) Define $\Omega = \Gamma \times S$ as the feature space, where $S$ is the set of nodes of interest and $\Gamma$ is the space of the graph structural data. We denote a point in $\Omega$ as $(\gG,S)$, where $\gG \in \Gamma$ is a graph and $S$ is a subset of nodes in $\gG$. $(\gG, S)$ is defined as a graph representation learning example, abbreviated as GRL example.

\textbf{Definition 2.6} (Graph isomorphism \& node isomorphism) Given two graphs $\gG^{(1)} = (A^{(1)}, X^{(1)}) $ and $\gG^{(2)} = (A^{(2)}, X^{(2)}) $. We call two GRL examples $(S^{(1)}, \gG^{(1)})$ and $(S^{(2)}, \gG^{(2)})$ are isomorphic if there exists a $\pi \in \Pi_n$, such that $A^{(1)} = \pi(A^{(2)})$, $X^{(1)} = \pi(X^{(2)})$ and $S^{(1)} = \pi(S^{(2)})$, denoted as $(S^{(1)}, \gG^{(1)}) \sim (S^{(2)}, \gG^{(2)})$. If the node set $S$ encloses all the nodes in $\gG$, it is called graph isomorphism. And if the node set $S$ corresponds to one single node in graph $\gG$, it is called node isomorphism.

To make predictions on graphs, we usually embed nodes into a low-dimensional space and then feed them into a classifier. Graph neural network \citep{bruna2013spectral, kipf2016semi, defferrard2016convolutional} is the most popular methods to learn node embeddings and message passing is the most prevalent framework to build GNNs\citep{gilmer2017neural}. Given a graph $\gG = (V,E,X)$, message passing framework uses node features and the graph structure to learn latent representation vectors of nodes in low dimension, by aggregating the node features through existing links:

1. Initialize node representations $\textbf{h}_v^{(0)}$ for $\forall v \in \gV$ as node features: $\textbf{h}_v^{(0)} \leftarrow X_v$.

2. Update node representations by aggregating the information through existing links. In $l-$th layer, we define a graph neural network layer as:

\begin{align}
\text{Message passing: }\quad &\textbf{m}_{uv}^{(l)} =  \phi_e(\textbf{h}_u^{(l-1)}, \textbf{h}_v^{(l-1)}), \forall (u,v) \in \gE \\
\text{Aggregation: }\quad &\textbf{a}_v{(l)} = \sum_{u \in \gN_v} (\textbf{m}_{uv}^{(l)}), \forall v \in \gV \\
\text{Update: }\quad &\textbf{h}_v^{(l)} = \phi_h(\textbf{h}_v^{(l-1)},\textbf{a}_v^{(l)})
\end{align}
Where $\gN_v$ represents the set of neighbours of node $v$. $\phi_e$ and $\phi_h$ are the node and edge operations which are usually implemented by neural networks. We abbreviate the message passing framework as MP-GNN in the following discussion.

MP-GNN extract latent representations for all the node in graph $\gG$, such that ${\textbf{h}_v| v \in \gV}$. The classifier depends on the specific prediction task, for example predicting potential links in a set of node pairs $\{(u,v) \in S|u \in \gv, v \in \gV\}$. The classifier is denoted as: 
\begin{align}
    \hat{y}_{S} = READOUT({\textbf{h}_u, \textbf{h}_v|(u,v)\in S})
\end{align}
Where the READOUT operation often be implemented by Multilayer Perceptron(MLP) or inner product. Combining the Eqs.(1)-(4), we can denote a GNN model built by MP-GNN as:
\begin{align}
    \hat{y}_{S} = f_{GNN}(\gG,S)
\end{align}

Since the graph structural data is intrinsically disordered, permutation equivariance is significant for GNN model. A fundamental request for GNN model is that the latent representations extracted by GNN should be equivariant to the order of nodes of the graph. To be more specific, when the node indices of a graph changes, the output of GNNs should do the same permutation actions. Luckily, MP-GNN satisfies permutation equivariance, which is proved in Appendix.


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Performance on ogb datasets, measured in Hit@20 and Hits@50 (mean$\pm$std\%). We run the codes on CPU: Intel(R) Xeon(R) Gold 6248R CPU @ 3.00GHz and GPU: NVIDIA QUADRO RTX 6000.\pan{what cpu? have SEAL precomputing time counts?}}
\scriptsize
\label{table2}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccc|cccc}
\hline
\multirow{3}{*}{Method} & \multicolumn{4}{c|}{ogbl-ddi}                           & \multicolumn{4}{c}{ogbl-collab}                         \\ \cline{2-9} 
                        & \multicolumn{4}{c|}{Hits@20(\%)}                        & \multicolumn{4}{c}{Hits@50(\%)}                         \\
                        & training time & test time & Validation   & test         & training time & test time & Validation   & test         \\ \hline
GCN                     & 29min 27s     & 0.20s     & 55.27 ± 0.53 & 37.11 ± 0.21 & 1h38min17s    & 1.38s     & 52.71 ± 0.10 & 44.62 ± 0.01 \\
SEAL                    & 2h 04min 32s  & 12.04s    & 28.29 ± 0.38 & 30.23 ± 0.24 & 2h29min05s    & 51.28s    & 64.95 ± 0.04 & 54.71 ± 0.01 \\
PGNN                    & 9min 49.39s   & 0.28s     & 2.66 ± 0.16  & 1.74 ± 0.19  & N/A           & N/A       & N/A          & N/A          \\
GNN-trans.              & 53min 26s     & 0.35s     & 15.63 ± 0.14 & 9.22 ± 0.21  & 1h52min22s    & 1.86s     & 18.17 ± 0.25 & 11.19 ± 0.42 \\ \hline
DW                      & 36min 41s     & 0.23s     & 0.04 ± 0.00  & 0.02 ± 0.00  & 34min40s      & 1.08s     & 53.64 ± 0.03 & 44.79 ± 0.02 \\
LE                      & 33min 42s     & 0.29s     & 0.09 ± 0.00  & 0.02 ± 0.00  & 37min22s      & 1.23s     & 0.10 ± 0.01  & 0.12 ± 0.02  \\ \hline
PEG-DW                  & 29min 56s     & 0.27s     & 56.47 ± 0.35 & 43.80 ± 0.32 & 1h42min 05s   & 1.43s     & 63.98 ± 0.05 & 54.33 ± 0.06 \\
PEG-LE                  & 30min 32s     & 0.29s     & 57.49 ± 0.47 & 30.16 ± 0.47 & 1h42min03s    & 1.42s     & 56.52 ± 0.12 & 48.76 ± 0.92 \\
PEG-DW+                 & 48min 03s     & 0.28s     & 59.70 ± 6.87 & 47.93 ± 0.21 & 1h37min43s    & 1.43s     & 62.31 ± 0.19 & 53.71 ± 8.02 \\
PEG-LE+                 & 51min 25.35s  & 0.29s     & 58.44 ± 7.46 & 32.33 ± 0.14 & 1h33min29s    & 1.39s     & 52.91 ± 1.24 & 45.96 ± 9.98 \\ \hline
\end{tabular}}
\end{table}



}

==> oldmodel.tex <==
The idea to achieve PE-stability is to set the GNN layer invariant to the positional features  given by the all possible bases of the entire eigenspace instead of some particular basis, because the eigenspace is much more stable. So, we propose PE-stable GNN layers as follows.
\begin{definition}[PE-stable GNN layers]
A PE-stable GNN layer that uses positional features $PE(A)$ satisfies $g(A, X, \text{PE}(A)) = g(A, X, \text{PE}(A)Q)$.
\end{definition}


Based on Thm.\ref{thm:stable}, we may prove the PE-stability of a PE-stable GNN layer, summarized in the following Thm. 

\begin{theorem} \label{thm:stable}
For two graphs 
\end{theorem}




%The above analysis shows the risk of using PE in a GNN layer. The issue is that eigenvectors given by EVD may not be stable when there are small eigengaps. However, a much stabler  of eigenvectors is      



Any two eigenvalues that are close may 



%\in \{-1,1,0\}^{Q\times Q}$ 



Previous works~\citep{dwivedi2020generalization,kreuzer2021rethinking} use LE to build graph transformers. Their GNN layers can be written as $g_{TF}(A, X, Z_{LE}) = g_{TF}(A, X+ \text{MLP}(Z_{LE}))$. 




%$Z^{(i)} = \text{PE}(A^{(i)})$, $i\in\{1,2\}$,



We say this GNN layer is stable if for any two graphs $\gG^{(1)}=(A^{(1)}, X^{(1)})$ and $\gG^{(2)} = (A^{(2)}, X^{(2)})$, letting $P^{*} = P^{*}(\gG^{(1)}, \gG^{(2)})$ denote their matching, then for some constant $C$, 
\begin{align} \label{eq:PE-stability}
    \| g(A^{(1)}, X^{(1)};W) - P^*g(A^{(2)}, X^{(2)};W)\| \leq Cd(\gG^{(1)}, \gG^{(2)})
\end{align}



PE is also termed graph/network embedding and often gives a way of dimension reduction of the graph structure~\citep{}.

Specifically, given a graph $\gG = (A, X)$ with $N$ nodes, PE works on $A$ and gives $Z=\text{PE}(A)\in\mathbb{R}^{N\times p}$ where each row $Z_v$ gives the positional feature of node $v$.







permutation equivariance is defined as
\begin{align}
   \text{Permutation Equivariance:}\quad Pg(A,H_i;W) = g(PAP^T,PH_i;W), \quad \forall P\in \Pi.
\end{align}



i.e., $Pg(A,H_i;W) = g(PAP^T,PH_i;W)$. 


Actually, this is a weaker condition of stability which is defined as follows

\begin{definition}[Permutation Equivariance]
If $H_o = g(A,H_i;W)$, then for any $P\in \Pi$, $PH_o = g(PAP^T,PH_i;W)$.
\end{definition}


\subsection{Positional Encoding, Uniqueness and Sensitivity}
The idea of positional encoding (PE) is to associate each node in the graph with a dense vector in some metric space where the distance between two vectors can approximate the distance between their corresponding nodes in the graph. Notationally, given a graph $\gG = (A, X)$ with $N$ nodes, PE works on $A$ and gives $Z=\text{PE}(A)\in\mathbb{R}^{N\times p}$ where each row $Z_v$ gives the positional feature of node $v$. PE is also termed graph/network embedding and often gives a way of dimension reduction of the graph structure~\citep{}.
%the vector characterizes the position of a node in the graph

Many PE techniques are actually based on optimization over the space of low-rank matrices. For example, Laplacian eigenmap (LE)~\citep{belkin2003laplacian}, $Z_{LE}$ includes the eigenvectors that correspond to the $p$ small eigenvalues of the Laplacian matrix $ L \triangleq D - A$ (or the normalized Laplacian matrix $ L_N \triangleq I-D^{-\frac{1}{2}}AD^{-\frac{1}{2}})$). Equivalently, letting $\tilde{L} = L$ or $ L_N$,
\begin{align*}
    Z_{LE} = \argmin_{Z\in\mathbb{R}^{N\times p}} \text{tr}(\tilde{L}ZZ^T),\quad \text{s.t.}\; Z^TZ = I.%\, \text{where $\tilde{L} = L (\triangleq D - A)$ or $ L_N (\triangleq I-D^{-\frac{1}{2}}AD^{-\frac{1}{2}})$.} 
\end{align*}
Other PE techniques, such as Deepwalk~\citep{}, Node2vec~\citep{}, LINE~\citep{} and PTE~\citep{} can be similarly unified into a low-rank matrix optimization form, where the corresponding $Z$ solves
\begin{align*}
 \min_{Z\in\mathbb{R}^{N\times p}} \text{tr}(f_+(A)g(ZZ^T) + f_-(D) g(-ZZ^T))
\end{align*}
Here $f_+(\cdot)$ revises $A$ by combining degree normalization and a power series of $A$, $f_-(A)$ corresponds to edge negative sampling and $g(\cdot)$ is a component-wise log-sigmoid function $x - \log(1+\exp(x))$. Specifically, in LINE, $f_+(A) = A$, $f_-(D) = c D^{\frac{3}{4}}$, for some positive constant $c$. For other PE techniques, the choice of $f_+$ and $f_-$ are listed in Appendix~\ref{apd:PE-detail}.  

The general difficulty of using $Z$ in GNN  






\begin{figure}[t]
\begin{minipage}{0.67\textwidth}
\begin{algorithm}[H]
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
$\hat{A} \odot\text{PE}(A)\text{PE}(A)^T X$

\caption{A PE-stable GNN layer $g(A, X, \text{PE}(A))$ }\label{alg:RWBT}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
\begin{figure}[H]
    \flushright
    % \includegraphics[trim={1.8cm 12cm 18.2cm 4.15cm},clip,width=0.99\textwidth]{AW-issue.pdf}
    \includegraphics[width=0.99\textwidth]{AW-issue2.pdf}
    \vspace{-0.7cm}
    \caption{\footnotesize{The correlation between walks needs to be captured to learn this law.}}
    \label{fig:AW-issue}
\end{figure}
\end{minipage}
\vspace{-0.55cm}
\end{figure}







\begin{align*}
    f_+(A) = A, \quad f_-(D) = c D^{\frac{3}{4}}\; \text{for some positive constant $c$}.
\end{align*}
For other PE techniques, we specify $f_+$ and $f_-$ in Appendix~\ref{apd:PE-detail}.






Many PE techniques are actually based on low-rank matrix factorization. For example, Laplacian eigenmap (LE)~\citep{belkin2003laplacian}, $Z_{LE}$ includes the eigenvectors that correspond to the $p$ small eigenvalues of the Laplacian matrix $ L \triangleq D - A$ (or the normalized Laplacian matrix $ L_N \triangleq I-D^{-\frac{1}{2}}AD^{-\frac{1}{2}})$). Equivalently, $Z=Z_{LE}$ plus some diagonal matrix $\Lambda=\Lambda_{LE}$ solves  
\begin{align*}
    \min_{Z\in\mathbb{R}^{N\times p}, \Lambda\in\mathbb{R}^{p\times p} } \| Z\Lambda Z^T  - \hat{A}\|_F^2, \;\text{where $\hat{A} \triangleq D + A$ (or $\hat{A} \triangleq I + D^{-\frac{1}{2}}AD^{-\frac{1}{2}})$}.
\end{align*}
Other PEs, such as deepwalk, node2vec, Line and PTE can be unified into a matrix factorization formulation, where $Z$ is obtained by solving
\begin{align*}
    \min_{Z\in\mathbb{R}^{N\times p}} \text{tr}(f_+(A)g(ZZ^T)) + tr(f_-(A)g(-ZZ^T))
\end{align*}





network embedding 








includes the eigenvectors that correspond to the $p$ small eigenvalues of the Laplacian matrix $ L \triangleq D - A$ or the normalized Laplacian matrix $ L_N \triangleq I-D^{-\frac{1}{2}}AD^{-\frac{1}{2}})$.




be represented as 
\begin{align*}
    Z_{LAP} = \argmin_{Z\in\mathbb{R}^{N\times p}} \text{tr}(Z^T\tilde{L}Z),\quad \text{s.t.}\; Z^TZ = I,\, \text{where $\tilde{L} = L (\triangleq D - A)$ or $ L_N (\triangleq I-D^{-\frac{1}{2}}AD^{-\frac{1}{2}})$.} 
\end{align*}
which is equivalent to the eigen
\begin{align*}
    \argmin_{M} \text{tr}(\tilde{L}M), \quad \text{s.t.} $$
\end{align*}

 %\text{CN}(\hat{Z}_{LAP}), \quad \text{where}\;\hat{Z}_{LAP} = \argmin_{Z\in\mathbb{R}^{N\times p}} \| Z^T Z - \hat{A}\|_F^2
where $\text{CN}(\cdot)$ is column-wise normalization and $\hat{A}$ denotes the negative normalized Laplacian with some bias.  


%many previous works focus on diminishing the above approximation error~\cite{}. 




%In practice, PE can also be viewed as a dimension reduction of the graph structure. 



how to dini   

a graph structure into a  



Given a graph $\gG = (A, X)$ with $N$ nodes, positional encoding (PE) is an operation that transforms the network structure $A$ into $Z=\text{PE}(A)\in\mathbb{R}^{N\times p}$ where each row. A GNN layer that uses PE will take $A, X, Z$ as the input and yield $H\in \mathbb{R}^{N\times q}$ as the output, where each row of $H$ can be viewed as the updated node representation 

\begin{definition}[Stability]
Consider two graphs $\gG_1 = (A_1, X_1)$ and $\gG_2 = (A_2, X_2)$ with $n$ nodes. A stable GNN layer that uses PE can be defined as $f:$
\end{definition}

is a computation $Z = \text{PE}(A)$.  



GNNs that utilize positional encoding  

\begin{align*}
    Given two graph
\end{align*}
















In this section we present Transferrable Positional Encoding Graph Neural Networks(PE-GNNs). Considering the permutation equivariance discussed in the former section, we claim that a powerful GNN model should satisfy the following:

\textbf{Conjecture 3.1} Given two isomorphic GRL examples $(S^{(1)}, \gG^{(1)}) \sim (S^{(2)}, \gG^{(2)})$, a good GNN model $f_{GNN}$ should make the same predictions, such that $f_{GNN}(S^{(1)}, \gG^{(1)}) = f_{GNN}(S^{(2)}, \gG^{(2)})$.

To meet this request, we must ensure both the GNN model and the READOUT classifier are permutation equivariant.

\subsection{Positional encodings}
MP-GNN can extract latent representations of nodes effectively, but it still has some limitations. Though it can not distinguish only a few graph structures, the applicability of GNNs in many real-word applications is limited. For example, it cannot distinguish structurally isomorphic nodes. (Figure 1)

To address this concern, some authors\citep{murphy2019relational} propose a GNN framework which assigns to each node an identifier that depends on the index ordering. However, using index ordering is computationally expensive since it requires to take all n! node permutations into consideration, thus requiring some sampling in practice. In this work, we keep the overall MP-GNN architecture and inject positional features to the nodes during the process of message passing. The positional features should be similar when the nodes are nearby on the graph, while the nodes far away from each other should have different positional features. Thus, the positional features could be defined as:

\textbf{Theorem 3.2} Given a graph $\gG$ with $n \times n$ adjacent matrix $A$, we define $Z$ as the positional features of graph $\gG$, if:
\begin{align}
ZZ^T & =M^* \\
M^* & = argminL(A,M)
\end{align}

Where $M$ is the low rank representations of the adjacent matrix $A$ and the rank could be defined arbitrarily from 1 to n. $L$ is the loss function, which is defined by the type of positional features.



\begin{figure}[htbp]
\begin{center}

\includegraphics[width=0.95\textwidth]{iclr2022/isomorphic_node.png}

\end{center}
\caption{In a node classification task, GNN cannot distinguish nodes $v_1$ and $v_2$ and classify them into different classes based on the graph structure alone.(Note we do not consider node features here) Node $v_1$ is labeled A and node $v_2$ is labeled B. GNN is expected to embed them into different point in the Euclidean Space. However, as the two nodes are isomorphic
in the graph, and their GNN corresponding subtrees used for message
aggregation are the same, GNNs will always assign the same embedding to both nodes no matter how deep the models are. Therefore, we can break the symmetry by adding positional features to each node and nodes $v_1$ and $v_2$ can thus be distinguished.}
\label{Fig3}
\end{figure}

The adjacency matrix could represent the structure of the graph, where rows and columns are correspond to nodes. Factorization-based methods are based on the matrix factorization approaches and are aimed to map row vectors and column vectors into the low-rank spaces. Thus, positional features could be obtained by matrix factorization methods. Graph Laplacian eigenvectors (LAP) \citep{belkin2003laplacian} is a factorization-based method which can embed the graphs into the Euclidean space. Specifically, LAP shows the locality over the graph and thus can better describe the distance between nodes, while preserving the global graph structure. Mathematically, LAP is defined via the factorization of the graph Laplacian matrix:

\begin{align}
    \Delta = I - D^{-\frac{1}{2}}AD^{-\frac{1}{2}} = U^T\Lambda U
\end{align}
Where $A$ is the $n \times$ n adjacent matrix, $D$ is the degree matrix, and $U$, $\Lambda$ are the eigenvectors and eigenvalues. Therefore, the LAP positional features can be obtained by the loss function:
\begin{align}
    M^* = argmin||M-\Delta||_F^2
\end{align}
Where $||\cdot||_F$ denotes Frobenius norm.

Except for factorization-based methods, the random walk based methods can also extract positional features. They utilize the random walks on graphs to approximate nodes' properties, such as centrality and similarity. Two far apart nodes has quite different random walk results, whereas two nearby nodes has similar random walk results. DeepWalk\citep{perozzi2014deepwalk} is the most commonly used random walk based method, which consists of 3 steps: (1)Sampling: Perform a few random walks from each node. To the best of our prior knowledge, it is sufficient to perform from 32 to 64 random walks from each node. (2)Training skip-gram:  Input each node from the random walk as a one-hot vector to the skip-gram network and maximizes the probability for predicting neighbor nodes. (3)Computing embeddings: Embedding is the output of a hidden layer of the skip-gram network. DeepWalk computes embeddings for each node. The loss function of DeepWalk can be denoted as:
\begin{align}
    M^* = argmin(cross-entropy(A,M))
\end{align}
Where 

The positional features for each node should be unique, otherwise it may not
distinguish isomorphic nodes which have same local neighbour graph structure and same positional features. For Graph Laplacian eigenvectors, although the eigenvectors are defined up to the factor ±1, we can fix it by designing specific structure in the model. For DeepWalk, we need to add some nuclear norm. Empirically it does not really matter.

Injected with positional features, we can state Conjecture 3.1 more explicitly:

\textbf{Remark 3.2} Given two isomorphic GRL examples $(S^{(1)}, \gG^{(1)}) \sim (S^{(2)}, \gG^{(2)})$. To be more specific, we can call them as $(S^{(1)}, A^{(1)},X^{(1)},Z^{(1)})$ and $(S^{(2)}, A^{(2)},X^{(2)},Z^{(2)})$, where $A$ is the adjacent matrix, $X$ is the node feature and $Z$ is the positional feature. Then we denote the GNN model as$f_{GNN}(S^{(i)}, G^{(i)} = READOUT(S^{(i)}, GNN(A^{(i)},X^{(i)}),Z^{(i)})$. A good GNN model $f_{GNN}$ should make the same predictions, such that $f_{GNN}(S^{(1)}, \gG^{(1)}) = f_{GNN}(S^{(2)}, \gG^{(2)})$.

\pan{We need to characterize the condition of the positional encodings that we are considering: 1. We need to have a unique low-rank matrix representation (which laplacian naturally satisfies while deepwalk may need to add some nuclear norm. Empirically it does not really matter. I can teach you this.); 2. positional encodings are obtained by factorizing such matrix representation.}

\subsection{PE-GNN}
There are two ways to make the model inductive. Firstly, the model architecture could be designed to support specific types of data. For example, convolution neural network (CNN) \citep{lecun1995convolutional} are designed to process image data and recurrent neural networks (RNN) \citep{hochreiter1998vanishing} are designed to process time series. These two types of data hold translation invariance in time and space. Thus, CNN and RNN have their parameters shared across space and time, in order to hold the invariance on the parameter level. Secondly, data argumentation could be adopted to cover all possible situations and thus can make the model inductive. For instance, Graph transformer \citep{dwivedi2020generalization} utilize LAP as positional features to capture the graph topology. However,  the laplacian eigenvectors are defined up to the factor ±1, therefore, they randomly flip the sign of eigenvectors in the training stage. As for graph structure data, we need to consider permutation equivariance since the node indices might be assigned differently. Besides, as the GNN embed each node of the graph into Euclidean space, isomorphic GRL examples may have their nodes in different position, while the relative distance between each node is the same. So we claim that a powerful GNN model should also hold position equivariance.  In the PE-GNN, we design the model inductive in the parameter level, which means the model is both permutation equivariant and position equivariant.

\textbf{Definition 3.3} (Position equivariance) Given a graph $\gG = (A,X,Z)$, where $A$ is the adjacent matrix, $X$ is the node feature and $Z$ is the positional feature. We denote the GNN model as $GNN(A,X,Z) = [\textbf{h}^{(k)},\textbf{z}^{(k)}]$. For $\forall Q \in O(n)$, where $O(n)$ is the orthogonal group. For $GNN(A,X,Z) = [\textbf{h}_1^{(k)},\textbf{z}_1^{(k)}]$ and $GNN(A, X, ZQ) = [\textbf{h}_2^{(k)},\textbf{z}_2^{(k)}]$. If $\textbf{z}_1^{(k)}Q = \textbf{z}_2^{(k)}$, we call the GNN model position equivariant.

Following the notations from preliminaries 2, we consider a graph $\gG = (\gV,\gE)$ with nodes $v_i \in \gV$. In addition to the node representation $\textbf{h}_i$, we also take positional features $\textbf{z}_i$ associated with each node into consideration. PE-GNN will preserve permutation equivariance on the set of nodes $\gV$ and also preserve position equivariance to the node position in the Euclidean space.

Inspired by the previous observation, we simplify the framework by adopting EGNN \citep{satorras2021n}. EGNN is designed for solving 3D translation and rotation symmetries, while our focus concentration is permutation equivariance and orthogonal group equivariance. Our Transferrable Positional Encoding Graph Convolution Layer (PEGCL) takes the node embeddings $\textbf{h}^l = \{\textbf{h}_0^l,...,\textbf{h}_{M-1}^l\}$ and the positional features $\textbf{z}^l = \{\textbf{z}_0^l,...,\textbf{z}_{M-1}^l\}$ as input, and outputs $\textbf{h}^{l+1}$ and $\textbf{x}^{l+1}$. The layer is defined mathematically as following:

\begin{align}
    \textbf{m}_{ij} &= \phi_e(||\textbf{x}_i^l - \textbf{x}_j^l||^2) \frac{e_{j,i}}{\sqrt{\hat{d}_i \hat{d}_j}} \textbf{h}_j^l \\
    \textbf{z}_i^{l+1} &= \textbf{z}_i^l \\
    \textbf{m}_i &= \sum_{j \in \gN(i) \cup\{i\}}\textbf{m}_{ij} \\
    \textbf{h}_i^{l+1} &= \phi_h(\textbf{m}_i)
\end{align}

Where $\hat{d}_i = 1+\sum_{j \in \gN(i)} e_{j,i}$ and $e_{j,i}$ denotes the edge weight from node $j$ to node $i$ (default:1.0). Notice we inject the positional features into the message passing process, and thus the model can capture the location information of nodes. The location information is crucial for tasks based on multiple nodes such as link prediction.

To predict potential links between a set of node-pairs $S$, we denote a readout layer as:
\begin{align}
    \hat{y}_s = \phi_{out}(\textbf{h}_u^T\textbf{h}_v, ||\textbf{x}_u^l - \textbf{x}_v^l||^2), (u,v) \in S
\end{align}

Our model is permutation equivariant on node indices for any permutation matrix $P$ and position equivariant on $z$ for any orthogonal matrix $Q \in O(n)$. More formally, our model satisfies:
$$
P\textbf{h}^{l+1}, P\textbf{z}^{l+1}Q = \text{PEGCL}(P\textbf{h}^l, P\textbf{z}^lQ)
$$
A formal proof of this is in Appendix. Therefore, our model is invariant to link prediction, as the readout function satisfies: 
$$
\text{READOUT}(\textbf{h}_u, \textbf{h}_v, \textbf{z}_u, \textbf{z}_v) = \text{READOUT}(\textbf{h}_u, \textbf{h}_v, \textbf{z}_uQ, \textbf{z}_vQ)
$$

(I think maybe it is not necessary to write introduction and theorem about expressive power. After all, I can only show that our model can distinguish isomorphic nodes, and thus have stronger expressive power than 1-WL test.)

GNN transformer also utilize positional features (LAP) to encode graph topology into the node features. Since LAP has multiplicity occuring due to the arbitrary sign of eigenvectors, they claim that they can fix the issue by  randomly flipping the sign of the eigenvectors during training stage. However, if the graph lapalacian eigenvalues don't differ from one another, the eigenvalues for each node are not unique, and thus the positional features for each node are not unique. GNN transformer doesn't work under this circumstance, but PE-GNN can work since we capture the relative distance $||\textbf{x}_i - \textbf{x}_j||$ between each node. Though some nodes may have different position features, but the relative distance between them is still. (The proof is in Appendix.) Therefore, PE-GNN is more powerful than GNN transformer.

\pan{Claim the issue of using the previous positional encodings: Different runs of algorithms may have different postional encodings. But the good thing is that the only difference between those encodings is just orthogonal group.}

\pan{Motivated by the previous observation. Show your general framework}

\pan{write theorem to show that your model is equivariant to the orthogonal group and thus invariant to for example link prediction}

\pan{We simplify the framework by adopting EGNN. Why I say it is a simplification. Because EGNN assume more than orthogonal group equivariance...}

\pan{Show case about the expressive power (perhaps can be removed)}

\pan{Show the issue of the GNN transformer by claiming the potential isotropic nodes in the graph.}
